PGADA: Perturbation-Guided Adversarial Alignment for Few-shot Learning Under the Support-Query Shift

Few-shot learning methods aim to embed the data to a low-dimensional embedding space and then classify the unseen query data to the seen support set. While these works assume that the support set and the query set lie in the same embedding space, a distribution shift usually occurs between the support set and the query set, i.e., the Support-Query Shift, in the real world. Though optimal transportation has shown convincing results in aligning different distributions, we find that the small perturbations in the images would significantly misguide the optimal transportation and thus degrade the model performance. To relieve the misalignment, we first propose a novel adversarial data augmentation method, namely Perturbation-Guided Adversarial Alignment (PGADA), which generates the hard examples in a self-supervised manner. In addition, we introduce Regularized Optimal Transportation to derive a smooth optimal transportation plan. Extensive experiments on three benchmark datasets manifest that our framework significantly outperforms the eleven state-of-the-art methods on three datasets.

==> experiment/bn.tex <==

\subsection{Effect of the Transductive Batch Normalization }
\label{appendix:tbncbn}
\input{table/bn}

Here, we explore the effect of transductive batch normalization (TBN)~\cite{bronskill2020tasknorm} and conventional batch normalization (CBN). TBN is first proposed in MAML~\cite{finn2017model}. Ren~\textit{et al.}\cite{ren2018meta} point out that TBN leverages a query set as a whole to bring a significant boost in performances compared to CBN. Therefore, we both deploy TBN and CBN to evaluate our method.  From Table~\ref{table:tbn_cbn}, we observe that PGADA gets unignorable benefit from TBN, which is consistent with prior works. Specifically, PGADA w/ TBN outperforms PGADA w/ CBN, $7.21\%$, $19.57\%$, $1.06\%$ on CIFAR100, miniImageNet, FEMNIST respectively. Once the self-supervised loss is removed, we observe that PGADA w/ TBN has a similar performance with PGADA w/ CBN.  It demonstrates that TBN and self-supervised learning can achieve better performance by exploring the inherent structure information from the unlabeled data.  Summing up, the prior works~\cite{finn2017model,triantafillou2019meta} point out that TBN is efficient in Meta-Learning, where TBN can explore whole query distribution cross tasks to achieve improvement. Our work obverse that the combination of TBN and self-supervised learning also performs well as they can learn more information from unlabeled data.  


==> experiment/case.tex <==
\subsection{Case Study}
\input{table/sqs}

Table~\ref{table:sqs} presents a case study to understand the effect of the support-query shift on CIFAR100 and miniImageNet. As mentioned in Sec.~\ref{sec:experiment_setup}, we strengthen the support-query shift by adopting different transformation functions on the support and query sets. We find that the support-query shift indeed significantly affects the behavior of PGADA, i.e., the performance drops by at least $40\%$ in both PGADA and TP. The decrease in performance shows the importance of this work in the real world. On the other hand, the performance of PGADA without the support-query shift also outperforms that of TP since our framework learns a more robust feature extractor.  Summing up, PGADA can still provide promising performance despite the absence of the support-query shift, showing PGADA is a general framework for few-shot learning.

==> fig/SQS_FSL.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width= \linewidth]{figure/SQS_FSL.pdf}
  \caption{Illustration of Support-Query Shift in a 5-way 1-shot classification task, where the support and query set are embedded in different distributions, resulting in inadequacy of conventional few-shot learning methods.}
  \label{fig:sqs-fsl}
\end{figure}

==> related/ot.tex <==
\subsection{Optimal Transport} 
Optimal transport has been adopted to many machine leaning task, including distribution estimation~\cite{courty2016optimal}, alignment~\cite{wang2021zero}, and clustering~\cite{ye2017fast}. 
To effectively solve the optimal transport, Sinkhorn's iterative algorithm  and its variants~\cite{cuturi2013sinkhorn,knight2008sinkhorn} are proposed which applies iterative Bregman projection. Besides, several works adopt optimal transport to solve domain adaptation problems~\cite{courty2016optimal}. Court et al.~\cite{courty2016optimal} introduce a regularized unsupervised optimal transportation model to align the representations in the source and target domains. 
Wang et al.~\cite{wang2021zero} estimate an optimal transport between the distributions of the generated features and that of the real features.


==> table/bn.tex <==
\begin{table*}[t]\small
\resizebox{\columnwidth}{!}{%
    \centering
    \begin{tabular}{ c|c|c|c|c|c|c|c|c|c }
\hline
  \multirow{3}*{Dataset}  &  \multicolumn{4}{|c|}{CIFAR100} &  \multicolumn{4}{|c|}{miniImageNet} & 
  FEMNIST\\

    \cline{2-10}
    &
    \multicolumn{2}{|c|}{8-target} &
    \multicolumn{2}{|c|}{16-target}&
    \multicolumn{2}{|c|}{8-target} &
    \multicolumn{2}{|c|}{16-target}&
    1-target \\
    \cline{2-10}
    & 1-shot& 5-shot & 
      1-shot& 5-shot & 
      1-shot& 5-shot & 
      1-shot& 5-shot & 
      1-shot \\
  \hline
  
  PGADA w/ TBN &  
 $\mathbf{42.16_{\pm 0.52}}$ &          $\mathbf{56.52_{\pm0.47}}$ &
 $\mathbf{42.73_{\pm 0.46}}$ & $\mathbf{56.83_{\pm0.40}}$ &
 $\mathbf{55.44_{\pm0.61}}$ &  $\mathbf{67.34_{\pm0.49}}$ &
 $\mathbf{55.69_{\pm0.62}}$ &  $\mathbf{66.90_{\pm0.50}}$ &
 $\mathbf{97.71_{\pm0.42}}$ \\
  
  PGADA w/ CBN & 
  $39.23_{\pm0.50}$ &
  $52.78_{\pm0.47}$ & 
  $39.75_{\pm0.45}$ & 
  $52.96_{\pm0.41}$ &
  $45.31_{\pm0.56}$ & 
  $57.42_{\pm0.48}$ &
  $45.63_{\pm0.50}$ & 
  $57.34_{\pm0.43}$ &
  $96.12_{\pm0.54}$ \\

%   PGADA$\dagger$ w/ TBN &   
%   $39.33_{\pm0.50}$& $53.66_{\pm0.47}$ &
%   $40.31_{\pm0.44}$& $54.23_{\pm0.40}$&
%   $47.96_{\pm0.57}$& $61.38_{\pm0.49}$&
%   $48.70_{\pm0.52}$& $61.44_{\pm0.43}$&
%   $96.53_{\pm0.52}$ \\


%     PGADA$\dagger$ w/ CBN &  
%  $39.72_{\pm0.51}$ &          
%  $53.18_{\pm0.46}$ &
%  $40.24_{\pm0.45}$ & 
%  $53.57_{\pm0.40}$ &
%  $48.44_{\pm0.59}$ &  
%  $60.91_{\pm0.50}$ &
%  $48.89_{\pm0.54}$ &  
%  $60.80_{\pm0.44}$ &
%  $96.03_{\pm0.55}$ \\
 
\hline    
\end{tabular}%
}
    \caption{Comparsion of TBN and CBN under the support-query shift. }
\label{table:tbn_cbn}
\end{table*}
% $\dagger$ means without self-supervised  loss.

==> table/sqs.tex <==
\begin{table*}[t]\small
\resizebox{\columnwidth}{!}{%
    \centering
    \begin{tabular}{ cc|c|c|c|c|c|c|c|c }
\hline
  \multicolumn{2}{c}{\multirow{3}*{Dataset}}  &  \multicolumn{4}{|c|}{CIFAR100} &  \multicolumn{4}{c}{miniImageNet} \\
    \cline{3-10}
    &&
    \multicolumn{2}{c|}{8-target} &
    \multicolumn{2}{c|}{16-target}&
    \multicolumn{2}{c|}{8-target} &
    \multicolumn{2}{c}{16-target} \\
    \cline{3-10}
    && 1-shot& 5-shot & 
      1-shot& 5-shot & 
      1-shot& 5-shot & 
      1-shot& 5-shot \\
 \hline

 \multirow{2}*{w/ SQS } & PGADA &  
  
    $42.16_{\pm 0.52}$ & $56.52_{\pm0.47}$ &
    $42.73_{\pm 0.46}$ & $56.83_{\pm0.40}$ &
    $55.44_{\pm 0.61}$ & $67.34_{\pm0.49}$ &
    $55.69_{\pm 0.62}$ & $66.90_{\pm0.50}$ \\
 
    & TP & 
    $34.00_{\pm0.46}$ & $49.71_{\pm0.47}$ & $35.55_{\pm0.41}$ & $50.24_{\pm0.39}$ &
    $40.49_{\pm0.54}$ & $59.85_{\pm0.49}$ &
    $43.83_{\pm0.51}$& $55.87_{\pm0.42}$  \\
     \hline
    \multirow{2}*{w/o SQS } & PGADA & 
    $90.32_{\pm0.18}$ &
    $94.26_{\pm0.17}$ & 
    $84.61_{\pm0.20}$ & 
    $87.24_{\pm0.19}$ &
    $86.83_{\pm0.27}$ & 
    $83.58_{\pm0.27}$ &
    $81.46_{\pm0.27}$& 
    $79.75_{\pm0.28}$ \\
  

    & TP & 
    $85.67_{\pm0.26}$ &
    $88.52_{\pm0.17}$ & 
    $82.40_{\pm0.20}$ & 
    $84.15_{\pm0.17}$ &
    $64.27_{\pm0.39}$ & 
    $75.22_{\pm0.30}$ &
    $69.68_{\pm0.59}$& 
    $72.67_{\pm0.52}$ \\

\hline    
\end{tabular}%
}
\caption{The case study of the support-query shift.}
\label{table:sqs}
\end{table*}
